A Multi-Type Multi-Span Network for Reading Comprehension that Requires Discrete Reasoning

Rapid progress has been made in the field of reading comprehension and question answering, where several systems have achieved human parity in some simplified settings. However, the performance of these models degrades significantly when they are applied to more realistic scenarios, such as answers involve various types, multiple text strings are correct answers, or discrete reasoning abilities are required. In this paper, we introduce the Multi-Type Multi-Span Network (MTMSN), a neural reading comprehension model that combines a multi-type answer predictor designed to support various answer types (e.g., span, count, negation, and arithmetic expression) with a multi-span extraction method for dynamically producing one or multiple text spans. In addition, an arithmetic expression reranking mechanism is proposed to rank expression candidates for further confirming the prediction. Experiments show that our model achieves 79.9 F1 on the DROP hidden test set, creating new state-of-the-art results. Source code\footnote{\url{https://github.com/huminghao16/MTMSN}} is released to facilitate future work.

==> sections/error_analysis.tex <==
\begin{table*}[!t]
\centering
\footnotesize
\begin{tabular}{lcllcc} %p{1cm}p{1cm}}
\toprule
Error Type & (\%) & Passage Snippets & Question & Answer & Prediction \\
 \midrule
 \midrule
\tabincell{c}{Arithmetic \\ computation} & 
38 &
\multicolumn{1}{m{4.5cm}}{\ldots{} there were 256,644 people living in Northern Cyprus. \ldots{} 2,482 born in the UK \ldots} & 
\multicolumn{1}{m{4.5cm}}{How many people in Northern Cyprus were not born in the UK?} & 
254,162 & 
144,923 \\
 \midrule
Sorting & 
18 &
\multicolumn{1}{m{4.5cm}}{\ldots{} 56.2\% were between the ages of 18 and 24; 16.1\% were from 25 to 44; 10.5\% were from 45 to 64 \ldots} & 
\multicolumn{1}{m{4.5cm}}{Which age group had the most people?} & 
\tabincell{c}{18 and \\ 24} & 
\tabincell{c}{from 45 \\ to 64} \\
 \midrule
\tabincell{c}{Multi-span \\ extraction} & 
13 &
\multicolumn{1}{m{4.5cm}}{Montana finished the regular season with \ldots{} 18 touchdowns, \ldots{} Craig was also a key contributor, \ldots{} and 10 touchdowns \ldots} & 
\multicolumn{1}{m{4.5cm}}{Which players scored ten or more touchdowns?} & 
\tabincell{c}{Craig, \\ Montana} & 
\tabincell{c}{Craig, \\ Rice} \\
 \midrule
\tabincell{c}{Single-span \\ extraction} & 
10 &
\multicolumn{1}{m{4.5cm}}{\ldots{} The sector decreased by 7.8 percent in 2002, before rebounding in 2003 with a 1.6 percent growth rate.} & 
\multicolumn{1}{m{4.5cm}}{In what year did the service sector have a sharp drop in growth rate?} & 
\tabincell{c}{2002} & 
\tabincell{c}{2003} \\
 \midrule
Counting & 
8 &
\multicolumn{1}{m{4.5cm}}{\ldots{} Macedonians with 338,358 inhabitants, Albanians with 103,891 \ldots{} Roma people with 23,475, Serbs (14,298 inhabitants) \ldots} & 
\multicolumn{1}{m{4.5cm}}{How many of the ethnic groups listed had more than 10,000 inhabitants in Skopje in 2002?} &
4 & 
3 \\
 \midrule
Span number & 
8 &
\multicolumn{1}{m{4.5cm}}{\ldots{} Tamil people form the majority of Chennais population. \ldots{} Chennais population was 80.7\% Hindu, 9.5\% Muslim \ldots} & 
\multicolumn{1}{m{4.5cm}}{Which religious people are the most common in Chennai?} & 
Hindu & 
\tabincell{c}{Hindu \\ Tamil} \\
\midrule
Other & 
5 &
\multicolumn{1}{m{4.5cm}}{\ldots{} 521,938 (6.6\%) of the economically active were unemployed \ldots} & 
\multicolumn{1}{m{4.5cm}}{How many in percent of the economically active were employed ?} & 
93.4 & 
48.4 \\
 \bottomrule
\end{tabular}
\caption{Error analysis on the DROP dev set. 100 randomly-sampled examples are classified into 7 categories. We list the error type, the ratio of each category, some representative examples, and our erroneous predictions.}
\label{tab:error_analysis}
\end{table*}
